Emergence of Segmentation with Minimalistic White-Box Transformers

Transformer-like models for vision tasks have recently proven effective for a wide range of downstream applications such as segmentation and detection. Previous works have shown that segmentation properties emerge in vision transformers (ViTs) trained using self-supervised methods such as DINO, but not in those trained on supervised classification tasks. In this study, we probe whether segmentation emerges in transformer-based models solely as a result of intricate self-supervised learning mechanisms, or if the same emergence can be achieved under much broader conditions through proper design of the model architecture. Through extensive experimental results, we demonstrate that when employing a white-box transformer-like architecture known as CRATE, whose design explicitly models and pursues low-dimensional structures in the data distribution, segmentation properties, at both the whole and parts levels, already emerge with a minimalistic supervised training recipe. Layer-wise finer-grained analysis reveals that the emergent properties strongly corroborate the designed mathematical functions of the white-box network. Our results suggest a path to design white-box foundation models that are simultaneously highly performant and mathematically fully interpretable. Code is at \url{https://github.com/Ma-Lab-Berkeley/CRATE}.

==> math_commands.tex <==
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{cleveref}


\newcommand{\myparagraph}[1]{\smallskip\noindent\textbf{#1.}}
\newcommand{\myparagraphit}[1]{\smallskip\noindent\textit{#1.}}


% Unary operators
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\Unif}{Unif}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\proj}{proj}

% Paired operators
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\parens}{\lparen}{\rparen}
\DeclarePairedDelimiter{\braces}{\{}{\}}
\DeclarePairedDelimiter{\brackets}{[}{]}


% Caligraphic
\newcommand\calA{{\mathcal{A}}}
\newcommand\calB{{\mathcal{B}}}
\newcommand\calC{{\mathcal{C}}}
\newcommand\calD{{\mathcal{D}}}
\newcommand\calE{{\mathcal{E}}}
\newcommand\calF{{\mathcal{F}}}
\newcommand\calG{{\mathcal{G}}}
\newcommand\calH{{\mathcal{H}}}
\newcommand\calI{{\mathcal{I}}}
\newcommand\calJ{{\mathcal{J}}}
\newcommand\calK{{\mathcal{K}}}
\newcommand\calL{{\mathcal{L}}}
\newcommand\calM{{\mathcal{M}}}
\newcommand\calN{{\mathcal{N}}}
\newcommand\calO{{\mathcal{O}}}
\newcommand\calP{{\mathcal{P}}}
\newcommand\calQ{{\mathcal{Q}}}
\newcommand\calR{{\mathcal{R}}}
\newcommand\calS{{\mathcal{S}}}
\newcommand\calT{{\mathcal{T}}}
\newcommand\calU{{\mathcal{U}}}
\newcommand\calV{{\mathcal{V}}}
\newcommand\calW{{\mathcal{W}}}
\newcommand\calX{{\mathcal{X}}}
\newcommand\calY{{\mathcal{Y}}}
\newcommand\calZ{{\mathcal{Z}}}


% Matrix
\newcommand\mA{{\boldsymbol{A}}}
\newcommand\mB{{\boldsymbol{B}}}
\newcommand\mC{{\boldsymbol{C}}}
\newcommand\mD{{\boldsymbol{D}}}
\newcommand\mE{{\boldsymbol{E}}}
\newcommand\mF{{\boldsymbol{F}}}
\newcommand\mG{{\boldsymbol{G}}}
\newcommand\mH{{\boldsymbol{H}}}
\newcommand\mI{{\boldsymbol{I}}}
\newcommand\mJ{{\boldsymbol{J}}}
\newcommand\mK{{\boldsymbol{K}}}
\newcommand\mL{{\boldsymbol{L}}}
\newcommand\mM{{\boldsymbol{M}}}
\newcommand\mN{{\boldsymbol{N}}}
\newcommand\mO{{\boldsymbol{O}}}
\newcommand\mP{{\boldsymbol{P}}}
\newcommand\mQ{{\boldsymbol{Q}}}
\newcommand\mR{{\boldsymbol{R}}}
\newcommand\mS{{\boldsymbol{S}}}
\newcommand\mT{{\boldsymbol{T}}}
\newcommand\mU{{\boldsymbol{U}}}
\newcommand\mV{{\boldsymbol{V}}}
\newcommand\mW{{\boldsymbol{W}}}
\newcommand\mX{{\boldsymbol{X}}}
\newcommand\mY{{\boldsymbol{Y}}}
\newcommand\mZ{{\boldsymbol{Z}}}

% Vectors
\newcommand\vzero{{\boldsymbol{0}}}
\newcommand\vone{{\boldsymbol{1}}}
\newcommand\vmu{{\boldsymbol{\mu}}}
\newcommand\vtheta{{\boldsymbol{\theta}}}
\newcommand\va{{\boldsymbol{a}}}
\newcommand\vb{{\boldsymbol{b}}}
\newcommand\vc{{\boldsymbol{c}}}
\newcommand\vd{{\boldsymbol{d}}}
\newcommand\ve{{\boldsymbol{e}}}
\newcommand\vf{{\boldsymbol{f}}}
\newcommand\vg{{\boldsymbol{g}}}
\newcommand\vh{{\boldsymbol{h}}}
\newcommand\vi{{\boldsymbol{i}}}
\newcommand\vj{{\boldsymbol{j}}}
\newcommand\vk{{\boldsymbol{k}}}
\newcommand\vl{{\boldsymbol{l}}}
\newcommand\vm{{\boldsymbol{m}}}
\newcommand\vn{{\boldsymbol{n}}}
\newcommand\vo{{\boldsymbol{o}}}
\newcommand\vp{{\boldsymbol{p}}}
\newcommand\vq{{\boldsymbol{q}}}
\newcommand\vr{{\boldsymbol{r}}}
\newcommand\vvs{{\boldsymbol{s}}}
\newcommand\vt{{\boldsymbol{t}}}
\newcommand\vu{{\boldsymbol{u}}}
\newcommand\vv{{\boldsymbol{v}}}
\newcommand\vw{{\boldsymbol{w}}}
\newcommand\vx{{\boldsymbol{x}}}
\newcommand\vy{{\boldsymbol{y}}}
\newcommand\vz{{\boldsymbol{z}}}

% Bold greek letters
\newcommand\balpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\bgamma{\boldsymbol{\gamma}}
\newcommand\bdelta{\boldsymbol{\delta}}
\newcommand\bepsilon{\boldsymbol{\epsilon}}
\newcommand\bzeta{\boldsymbol{\zeta}}
\newcommand\betaa{\boldsymbol{\eta}} % bold eta can not beta...
\newcommand\btheta{\boldsymbol{\theta}}
\newcommand\biota{\boldsymbol{\iota}}
\newcommand\bkappa{\boldsymbol{\kappa}}
\newcommand\blambda{\boldsymbol{\lambda}}
\newcommand\bmu{\boldsymbol{\mu}}
\newcommand\bnu{\boldsymbol{\nu}}
\newcommand\bxi{\boldsymbol{\xi}}

\newcommand\bpi{\boldsymbol{\pi}}
\newcommand\brho{\boldsymbol{\rho}}
\newcommand\bsigma{\boldsymbol{\sigma}}
\newcommand\btau{\boldsymbol{\tau}}
\newcommand\bupsilon{\boldsymbol{\upsilon}}
\newcommand\bphi{\boldsymbol{\phi}}
\newcommand\bchi{\boldsymbol{\chi}}
\newcommand\bpsi{\boldsymbol{\psi}}
\newcommand\bomega{\boldsymbol{\omega}}

\newcommand\bAlpha{\boldsymbol{\Alpha}}
\newcommand\bBeta{\boldsymbol{\Beta}}
\newcommand\bGamma{\boldsymbol{\Gamma}}
\newcommand\bDelta{\boldsymbol{\Delta}}
\newcommand\bEpsilon{\boldsymbol{\Epsilon}}
\newcommand\bZeta{\boldsymbol{\Zeta}}
\newcommand\bEta{\boldsymbol{\Eta}}
\newcommand\bTheta{\boldsymbol{\Theta}}
\newcommand\bIota{\boldsymbol{\Iota}}
\newcommand\bKappa{\boldsymbol{\Kappa}}
\newcommand\bLambda{\boldsymbol{\Lambda}}
\newcommand\bMu{\boldsymbol{\Mu}}
\newcommand\bNu{\boldsymbol{\Nu}}
\newcommand\bXi{\boldsymbol{\Xi}}
\newcommand\bPi{\boldsymbol{\Pi}}
\newcommand\bRho{\boldsymbol{\Rho}}
\newcommand\bSigma{\boldsymbol{\Sigma}}
\newcommand\bTau{\boldsymbol{\Tau}}
\newcommand\bUpsilon{\boldsymbol{\Upsilon}}
\newcommand\bPhi{\boldsymbol{\Phi}}
\newcommand\bChi{\boldsymbol{\Chi}}
\newcommand\bPsi{\boldsymbol{\Psi}}
\newcommand\bOmega{\boldsymbol{\Omega}}

% Sets
\newcommand\sA{{\mathbb{A}}}
\newcommand\sB{{\mathbb{B}}}
\newcommand\sC{{\mathbb{C}}}
\newcommand\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\newcommand\sE{{\mathbb{E}}}
\newcommand\sF{{\mathbb{F}}}
\newcommand\sG{{\mathbb{G}}}
\newcommand\sH{{\mathbb{H}}}
\newcommand\sI{{\mathbb{I}}}
\newcommand\sJ{{\mathbb{J}}}
\newcommand\sK{{\mathbb{K}}}
\newcommand\sL{{\mathbb{L}}}
\newcommand\sM{{\mathbb{M}}}
\newcommand\sN{{\mathbb{N}}}
\newcommand\sO{{\mathbb{O}}}
\newcommand\sP{{\mathbb{P}}}
\newcommand\sQ{{\mathbb{Q}}}
\newcommand\sR{{\mathbb{R}}}
\newcommand\sS{{\mathbb{S}}}
\newcommand\sT{{\mathbb{T}}}
\newcommand\sU{{\mathbb{U}}}
\newcommand\sV{{\mathbb{V}}}
\newcommand\sW{{\mathbb{W}}}
\newcommand\sX{{\mathbb{X}}}
\newcommand\sY{{\mathbb{Y}}}
\newcommand\sZ{{\mathbb{Z}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
\declaretheorem[numberwithin=section,style=plain]{theorem}
\declaretheorem[sibling=theorem,style=plain]{proposition}
\declaretheorem[sibling=theorem,style=plain]{lemma}
\declaretheorem[sibling=theorem,style=plain]{corollary}

% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
\declaretheorem[sibling=theorem,style=definition]
{definition}
\declaretheorem[sibling=theorem,style=definition]
{assumption}

% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}
\declaretheorem[sibling=theorem,style=remark]
{remark}

\crefname{lemma}{lemma}{lemmas}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{thm}{theorem}{theorems}
\Crefname{thm}{Theorem}{Theorems}
\crefname{assumption}{assumption}{assumptions}
\Crefname{assumption}{Assumption}{Assumptions}



\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\tvx}{\tilde{\vx}}
\newcommand{\tcalX}{\tilde{\calX}}
